Effects of Risk on Privacy Contracts for Demand-Side Management

As smart meters continue to be deployed around the world collecting unprecedented levels of fine-grained data about consumers, we need to find mechanisms that are fair to both, (1) the electric utility who needs the data to improve their operations, and (2) the consumer who has a valuation of privacy but at the same time benefits from sharing consumption data. In this paper we address this problem by proposing privacy contracts between electric utilities and consumers with the goal of maximizing the social welfare of both. Our mathematical model designs an optimization problem between a population of users that have different valuations on privacy and the costs of operation by the utility. We then show how contracts can change depending on the probability of a privacy breach. This line of research can help inform not only current but also future smart meter collection practices.

==> makefile <==
# set latexfile to the name of the main file without the .tex
latexfile = arxiv
# put the names of figure files here.  include the .eps
#figures = 
# if no references, run "touch latexfile.bbl; touch referencefile.bib"
# or delete dependency in .dvi and tarball sections
referencefile = 2014IEEETSG

TEX = pdflatex

# support subdirectories
VPATH = Figs


# idea from http://ctan.unsw.edu.au/help/uk-tex-faq/Makefile
#$(latexfile).dvi : $(figures) $(latexfile).tex 
$(latexfile).pdf : $(figures) $(latexfile).tex $(referencefile).bbl
	while ($(TEX) $(latexfile) ; \
	grep -q "Rerun to get cross" $(latexfile).log ) do true ; \
	done


# keep .eps files in the same directory as the .fig files
#%.eps : %.fig
#	fig2dev -L eps $< > $(dir $< )$@

# The command below makes pdf from ps, call "make pdf" to run
#$(latexfile).pdf : $(latexfile).ps
#	ps2pdf $(latexfile).ps $(latexfile).pdf

#pdf : $(latexfile).pdf

# The command blow makes ps from dvi, call "make ps" to run
#$(latexfile).ps : $(latexfile).dvi
#	dvips $(latexfile)

#ps : $(latexfile).ps 

# The command below creates a tarball, call "make tarball" to run
$(latexfile).tar.gz : $(figures) $(latexfile).tex $(referencefile).bib
	tar -czvf $(latexfile).tar.gz $^

tarball: $(latexfile).tar.gz

# short cuts for multiple runs, cpall compiles all, clean removes junk, bibit runs bibtex alone
cpall:
	make; make pdf; skim $(latexfile).pdf; rm $(latexfile).dvi $(latexfile).log 
	#$(latexfile).ps
clean:
	rm $(latexfile).dvi $(latexfile).log $(latexfile).ps $(latexfile).pdf

bibit: 
	bibtex $(latexfile)

mpdf:
	pdflatex $(latexfile).tex; skim $(latexfile).pdf

